The role of rare-earth atoms in the anisotropy and antiferromagnetic exchange coupling at a hybrid metal-organic interface

Magnetic anisotropy and magnetic exchange interactions are crucial parameters that characterize the hybrid metal-organic interface, key component of an organic spintronic device. We show that the incorporation of 4$f$ RE atoms to hybrid metal-organic interfaces of CuPc/REAu$_2$ type (RE= Gd, Ho) constitutes a feasible approach towards on-demand magnetic properties and functionalities. The GdAu$_2$ and HoAu$_2$ substrates differ in their magnetic anisotropy behavior. Remarkably, the HoAu$_2$ surface boosts the inherent out-of-plane anisotropy of CuPc, owing to the match between the anisotropy axis of substrate and molecule. Furthermore, the presence of RE atoms leads to a spontaneous antiferromagnetic (AFM) exchange coupling at the interface, induced by the 3$d$-4$f$ superexchange interaction between the unpaired 3$d$ electron of CuPc and the 4$f$ electrons of the RE atoms. We show that 4$f$ RE atoms with unquenched quantum orbital momentum ($L$), as it is the case of Ho, induce an anisotropic interfacial exchange coupling.

==> aux4_SM_magnetCuPc_REAu2_200224.tex <==


